Adversarial Bandits with Knapsacks

We consider Bandits with Knapsacks (henceforth, BwK), a general model for multi-armed bandits under supply/budget constraints. In particular, a bandit algorithm needs to solve a well-known knapsack problem: find an optimal packing of items into a limited-size knapsack. The BwK problem is a common generalization of numerous motivating examples, which range from dynamic pricing to repeated auctions to dynamic ad allocation to network routing and scheduling. While the prior work on BwK focused on the stochastic version, we pioneer the other extreme in which the outcomes can be chosen adversarially. This is a considerably harder problem, compared to both the stochastic version and the "classic" adversarial bandits, in that regret minimization is no longer feasible. Instead, the objective is to minimize the competitive ratio: the ratio of the benchmark reward to the algorithm's reward. We design an algorithm with competitive ratio O(log T) relative to the best fixed distribution over actions, where T is the time horizon; we also prove a matching lower bound. The key conceptual contribution is a new perspective on the stochastic version of the problem. We suggest a new algorithm for the stochastic version, which builds on the framework of regret minimization in repeated games and admits a substantially simpler analysis compared to prior work. We then analyze this algorithm for the adversarial version and use it as a subroutine to solve the latter.

==> DP-analysis.tex <==
\section{Analysis for dynamic pricing: proof of Theorem~\ref{thm:DP}}
\label{sec:DP-analysis}


==> LB-analysis.tex <==
\section{Analysis for the lower bounds: proof of Theorem~\ref{thm:LB-main}}
\label{sec:LB-analysis}

\xhdr{Notation.} Throughout this section we use the following notation. Given an instance $\mI$, we denote $\OPTFD(\mI)$, $\OPTFA(\mI)$ and $\OPTDP(\mI)$ to denote the optimal value of the best fixed distribution, best fixed arm and best dynamic policy respectively, for instance $\mI$. Likewise let $\OPTLPfull(\mI)$ denote the optimal $\LP$ value for instance $\mI$ and given an algorithm $\mA$ and an instance $\mI$, let $\E[\REW(\mA, \mI)]$ denote the expected reward obtained by $\mA$ on instance $\mI$, where the expectation is over the internal randomness of the algorithm.

	\xhdr{Proof of Lemma~\ref{lem:optfull-optfd}.} Before we proceed we first prove Lemma~\ref{lem:optfull-optfd}. Let $\tau^*$ denote the time-step at which $\OPTLPfull$ is maximized. Let $\vec{p}$ denote the optimal solution to $\tau^* \cdot \OPTLP(\bvM_{\tau^*}, B(1-\epsilon), \tau^*)$ where $\epsilon=\sqrt{\frac{\log dT}{B}}$. Note that $\OPTFD$ is at least as large as the expected total reward obtained by the distribution $\vec{p}$. From the Chernoff-Hoeffding bounds (Lemma~\ref{lem:Chernoff}), with probability at least $1-dT^{-2}$ we have
	
		\[
				\forall i \in [d] \qquad \sum_{t \in [\tau^*]} \vec{p} \cdot \vec{c}_{t, i} \leq B.
		\]
	
		Thus conditioning on this event the expected total reward obtained by $\vec{p}$ is $\sum_{t \in [\tau^*]} \vec{p} \cdot \vec{r}_t$ $=$ $\tau^* \cdot \OPTLP(\bvM_{\tau^*}, B(1-\epsilon), \tau^*)$. Thus the expected total reward obtained by $\vec{p}$ is at least $\tau^* \cdot \OPTLP(\bvM_{\tau^*}, B(1-\epsilon), \tau^*)$ \footnote{With probability $T^{-2}$ we assume that $\vec{p}$ has an expected reward of $0$.}. Moreover from \refeq{eq:scaledBudgetOPTVals1} we have that 
		
		\[
			\textstyle \tau^* \cdot \OPTLP(\bvM_{\tau^*}, B(1-\epsilon), \tau^*) \geq (1-\epsilon) \tau^* \cdot \OPTLP(\bvM_{\tau^*}, B(1-\epsilon), \tau^*).
		\]	
		
		Thus we have
			
			\begin{equation}
				\label{eq:lowerBdOPTFD}	
				\OPTFD \geq \tau^* \cdot \OPTLP(\bvM_{\tau^*}, B(1-\epsilon), \tau^*) \geq \OPTLPfull - O\Paren{\OPTLPfull \sqrt{\frac{\log dT}{B}}}.
			\end{equation}
	
	


\subsection{Warm-up: proof of Lemma~\ref{thm:simpleLowerBound}}
\label{sec:LB-warmup}
				
Denote the two arms by $A_1$ and $A_0$ where $A_0$ denotes the null arm. The consumption for arm $A_1$ is $1$ for all rounds in both $\mI_1$ and $\mI_2$. Thus the only difference between the two instances is the rewards obtained for playing arm $A_1$ in each round. The instances have two phases where each phase lasts for $\tfrac{T}{2}$ rounds. In phase $1$, in both $\mI_1$ and $\mI_2$ playing arm $A_1$ fetches a reward $\tfrac{1}{2}$. In the second phase, in $\mI_1$, the reward for playing arm $A_1$ is $0$ while in $\mI_2$ the reward for playing arm $A_1$ is $1$. Thus the \emph{outcome} matrix for the first $\tfrac{T}{2}$ time-steps is the same in instances $\mI_1$ and $\mI_2$.
			
			Consider a randomized algorithm $\mA$. Let $\alpha_1$ be the expected number of times arm $A_1$ is played by $\mA$ in the first $\tfrac{T}{2}$ rounds on instances $\mI_1$ and $\mI_2$. Note since the outcome matrix is same, the expected number of times the arm is played should be same in both the instances. Let $\alpha_{2, 1}$, $\alpha_{2, 2}$ denote the expected number of times arm $A_1$ is played in the second phase in instances $\mI_1$ and $\mI_2$ respectively.
			
			
			Recall that in this section we are interested in a lower-bound on the competitive ratio $\OPTFD/\E[\REW]$ for every instance. 
			
			
			Consider $\OPTLPfull(\mI_1)$, the optimal value of the best fixed distribution on $\mI_1$.  Using \refeq{eq:adv-stoppedLP} with $\tau=\tfrac{T}{2}$ this equals $\frac{T}{2} \cdot \OPTLP\Paren{\bvM_{\tfrac{T}{2}}, B, \tfrac{T}{2}}$ which evaluates to $\tfrac{T}{4}$.
			
			Likewise $\OPTLPfull(\mI_2)$ equals $T \cdot \OPTLP\Paren{\bvM_{T}, B, T}$, which evaluates to $\tfrac{3T}{4}$.
			
			
			
			Consider the performance of $\mA$ on $\mI_1$. We have,
			
			\begin{equation}
				\label{eq:simple-lower-cr1}
				\textstyle \tfrac{\OPTLPfull(\mI_1)}{\E[\REW(\mA, \mI_1)]} \geq \Paren{\tfrac{T}{4}}/\Paren{ \tfrac{\alpha_1}{2} }.
			\end{equation}
			
			Likewise on $\mI_2$ we have,
			
			\begin{equation}
				\label{eq:simple-lower-cr2}
				\textstyle \tfrac{\OPTLPfull(\mI_2)}{\E[\REW(\mA, \mI_2)]}  \geq \Paren{ \tfrac{3T}{8} }/\Paren{ \tfrac{\alpha_1}{2} + \alpha_{2, 2} }.	
			\end{equation}

			Thus the competitive ratio of $\mA$ is at least the maximum of the ratios in \refeq{eq:simple-lower-cr1} and \refeq{eq:simple-lower-cr2}. Thus we want to minimize this maximum and is achieved when the two ratios are equal to each other.
			
			Notice that the term $\alpha_{2, 1}$ does not appear in \refeq{eq:simple-lower-cr1} and \refeq{eq:simple-lower-cr2}. By setting the term in \refeq{eq:simple-lower-cr1} equal to the term in \refeq{eq:simple-lower-cr2} and re-arranging,
			
			\begin{equation}
				\label{eq:otherEq-simple-lower}
				\textstyle	\alpha_1 = 4 \alpha_{2, 2}.
			\end{equation}

			Moreover we have $\alpha_1 + \alpha_{2, 2} \leq B$. Combining this with \refeq{eq:otherEq-simple-lower} we get $\alpha_1 \leq \tfrac{4B}{5} = \tfrac{2T}{5}$ and the corresponding competitive ratio is at least $\Paren{ \tfrac{T}{4} }/\Paren{ \tfrac{\alpha_1}{2} } \geq \frac{5}{4}$.
			
			Moreover from \refeq{eq:lowerBdOPTFD} with $d=1$ we get that for every $j \in [2]$,
			\[
					\textstyle \OPTFD(\mI_j)/\E[\REW(\mA, \mI_j)] \geq \frac{5}{4} - O\Paren{\frac{\OPTLPfull}{T} \sqrt{\frac{\log T}{B}}}.
			\]
			
			Thus any randomized algorithm $\mA$ has a competitive ratio, defined as $\OPTFD/\E[\REW]$, of at least $\frac{5}{4} - o(1)$, since $B \geq \Omega(\log T)$.

	
	

\subsection{The main lower bound: proof of Lemma~\ref{lm:LB-main}}
\label{sec:LB-main}

Fix any randomized algorithm $\mA$. As before in this sub-section we are interested in the ratio $\OPTFD/\mathbb{E}[\REW(\mA)]$. We argue that it has the claimed competitive ratio on at least one instance $\mI_\tau$ in the construction~\ref{con:LB-main}. The proof proceeds in two parts. We first argue about the solution structure of the optimal distribution for the construction~\ref{con:LB-main} (we prove this formally in Lemma~\ref{lem:optimalSolutionLB}). Next we characterize the expected number of times arm $A_1$ is played if $\mA$  optimal algorithm in each of the phases. Combining the two we get Lemma~\ref{lm:LB-main}.

\xhdr{Structure of the optimal solution.} Define \(\OPTLP(\bvM_{\tau^*}, B, \tau^*)\) to be the optimal value of $\LP$~\ref{lp:primalAbstract} on the instance \(\mI_\tau\). Then we have the following Lemma.

	\begin{lemma}
		\label{lem:optimalSolutionLB}
		For a given instance $\mI_{\tau}$ we have the following.
		\begin{enumerate}
			\item The optimal stopping time $\tau^* = B \tau$.
			\item \(\OPTLP(\bvM_{\tau^*}, B, \tau^*) \leq \frac{1}{\tau}\sum_{t \in [B \tau]} \mP(t) \epsilon\).
		\end{enumerate}
	\end{lemma}
	
	\begin{proof}
	Note that (2) follows from (1). Indeed, given that the stopping time is $B\tau$, the optimal solution is to set $X(1) = \frac{1}{\tau}$ and $X(0) = 1-\frac{1}{\tau}$ thus obtaining a total reward of $\frac{1}{\tau} \sum_{t \in [B \tau]} \mP(t) \epsilon$. Thus it remains to prove (1). 
	
	First it is easy to prove that $\tau^* \leq B\tau$. Since there are no rewards after time-step $\tau^*$, we have
	\[
			\textstyle \forall t' > 0 \qquad  \OPTLP(\bvM_{\tau*+t'}, B, \tau^*+t') = \frac{1}{\tau+t'} \sum_{t \in [\tau^*]} \mP(t) \epsilon < \frac{1}{\tau} \sum_{t \in [B \tau]} \mP(t) \epsilon.
	\]
	
	Now we will argue that the optimal stopping time cannot be strictly lesser than $\tau^*$. To do so, first we argue that for two stopping times $t_1 < t_2$ within the same phase, the maximum objective is achieved for the stopping time $t_2$. This implies that the optimal stopping time has to be the last time step of some phase.
	
		Consider times $t_1 < t_2$ such that $\mP(t_1) = \mP(t_2) = \tau$. Then we want to claim that
		\[
			\textstyle \frac{B}{t_1} \Paren{\sum_{t \in [t_1]} \mP(t) \epsilon} \leq \frac{B}{t_2} \Paren{\sum_{t \in [t_2]} \mP(t) \epsilon}.
		\]	
		For contradiction assume the inequality does not hold. Then we have the following.
		
		\[
			\textstyle \sum_{t \in [t_1]} \mP(t) > \frac{t_1}{t_2} \Paren{\sum_{t \in [t_2]} \mP(t)}.
		\]
	
		Note that $\sum_{t \in [B(\tau-1)]}\mP(t) = \sum_{t' \in [\tau]} B t' = \frac{B(\tau-1)\tau}{2}$. Thus we have
		
		\begin{align*}
			\textstyle \sum_{t \in [t_1]} \mP(t) & \textstyle = \frac{B(\tau-1)\tau}{2} + (t_1-B(\tau-1))\tau,\\
			\textstyle \sum_{t \in [t_2]} \mP(t) & \textstyle = \frac{B(\tau-1)\tau}{2} + (t_2-B(\tau-1))\tau.
		\end{align*}
			
		Therefore we have,
		\[
			\textstyle \frac{B(\tau-1)\tau}{2} + (t_1-B(\tau-1))\tau > \frac{t_1B(\tau-1)\tau}{2t_2} + (t_2-B(\tau-1))\tau.
		\]
		
		Further re-arranging we have $\frac{B(\tau-1)}{2} > t_2$. This is a contradiction since $t_2$ is in phase $\tau$ and thus is at least $B(\tau-1)$.
	
		Next we argue that the optimal value is achieved when the stopping time is in the last \emph{non-zero rewards phase}. Consider two phases $\tau_1 < \tau_2$. Thus the ending times are $B \tau_1$ and $B \tau_2$. To prove that the optimal value increases by stopping at $B \tau_2$, as opposed to $B \tau_1$, we want to show that
		
		\[
				\textstyle \frac{1}{\tau_1} \sum_{t \in [\tau_1]} B t \epsilon \leq \frac{1}{\tau_2} \sum_{t \in [\tau_2]} B t \epsilon.
		\]
		
		As before assume for a contradiction that this doesn't hold. Then re-arranging we get,
		
		\[
			\textstyle	\frac{\tau_1(\tau_1 + 1)}{2} > \frac{\tau_1 (\tau_2 + 1)}{2}.
		\]
		
		Further re-arranging we get $\tau_1 > \tau_2$. This is a contradiction since $\tau_1 < \tau_2$. Thus these arguments imply that the stopping time $\tau^* = B\tau$.
	\end{proof}

\xhdr{Expected behavior of the optimal algorithm.} Consider any randomized algorithm $\mA$. The performance of $\mA$ is then as follows.

	\begin{equation}
		\label{eq:lowerBoundMain}
		\textstyle \tfrac{\OPTLPfull}{\E[\REW(\mA)]} \geq \max_{1 \leq \tau \leq T/B} \frac{B \tau \cdot \OPTLP(\bvM_{B\tau}, B, B \tau)}{\E[\REW(\mA)]}.
	\end{equation}
	
	Consider two consecutive instances \(\mI_{\tau}\) and \(\mI_{\tau+1}\). The outcome matrix in the phases $1, 2 \LDOTS \tau$ look identical in both these instances. Thus the expected number of times arm $A_1$ is chosen by algorithm $\mA$ in phases $1, 2 \LDOTS \tau$ is identical. Let \(\alpha_{\tau}\) denote the expected number of times $\mA$ plays arm \(A_1\) in phase \(\tau\) on instances $\mI_{1}, \mI_{2}, \LDOTS \mI_{\tau}$. The expected number of times arm \(A_1\) is played in phase \(\tau\) on instances $\mI_{\tau+1}, \mI_{\tau+2} \LDOTS \mI_{T/B}$ is set arbitrarily since this term does not appear in the objective function (\ie $\E[\REW(\mA)]$). Thus the maximum of the ratios in \refeq{eq:lowerBoundMain} occurs when they are equal for all values $\tau$. Therefore we want for every \(1 \leq \tau \leq T/B\),

	\begin{equation}
		\label{eq:EqualLowerBound}
		\textstyle \frac{\frac{1}{\tau} \sum_{j \in [\tau]} B j \epsilon}{\sum_{j \in [\tau]} j \epsilon \alpha_j} =  \frac{\frac{1}{\tau+1} \sum_{j \in [\tau+1]} B j \epsilon}{\sum_{j \in [\tau+1]} j \epsilon \alpha_j}.
	\end{equation}


Also note that \(\alpha_1 + \alpha_2 + \ldots + \alpha_{T/B} \leq B\), since the total budget is $B$ and the consumption is $1$ in every round for arm $A_1$ and $0$ for arm $A_0$. We will prove that these lead to the following recurrence for the maximizing values of
\(\alpha_j\).

\begin{equation}
	\label{eq:lowerBoundRecurrence}	
	\textstyle \forall j \geq 2 \qquad \alpha_j = \frac{1}{2j} \alpha_1.
\end{equation}

We will prove the recurrence \refeq{eq:lowerBoundRecurrence} via induction.
The base case is when \(j=2\). Plugging in $\tau=1$ in \refeq{eq:EqualLowerBound} we have

\[
	\textstyle \frac{1}{\alpha_1} = \frac{3/2}{\alpha_1 + 2\alpha_2}.
\]

This implies that \(\alpha_2 = \frac{1}{4}\alpha_1\). Therefore we are done. Now consider the inductive case; let all \(\alpha\) up to \(\alpha_{\tau}\) satisfy the recurrence \refeq{eq:lowerBoundRecurrence}. Consider the instance $\mI_{\tau}$ and $\mI_{\tau+1}$. From \refeq{eq:EqualLowerBound} we have,

\[
	 \frac{\frac{1}{\tau} \sum_{j \in [\tau]} jB}{\alpha_1 + \sum_{j=2}^\tau \alpha_1/2} =  \frac{\frac{1}{\tau+1} \sum_{j \in [\tau+1]} jB}{\alpha_1 + \sum_{j=2}^{\tau} \alpha_1/2 + (\tau+1) \alpha_{\tau+1}}.
\]

Rearranging, we get that
\(\alpha_{\tau+1} = \tfrac{1}{2(\tau+1)} \alpha_1\). This completes the inductive step.

Using the fact that
\(\alpha_1 (1 + 1/4 + 1/6 + \ldots + B/2T) \leq B\) we have that
\(\alpha_1 \leq \frac{B}{2H(T/B)} \) where $H(n)$ denotes the $n^{th}$ Harmonic number. The value of \refeq{eq:lowerBoundMain} for \(\tau=1\) is the same at all other \(\tau\) and has a value of \(\frac{B}{\alpha_1} \geq 2H\Paren{\tfrac{T}{B}} \geq \Omega\Paren{\log \frac{T}{B}} \geq \Omega\Paren{\log T}\). The second last inequality uses the well-known fact that $\zeta + \log n \leq H(n) \leq \zeta + \log (n+1)$ for an absolute constant $\zeta$ and the last inequality uses the fact that $B \in \Brac{\Omega(\log^3 T), O(T^{1-\alpha})}$.


	Therefore we have that for every instance $j \in \Brac{\frac{T}{B}}$,
	\[
			\textstyle \frac{\OPTLPfull(\mI_j)}{\E[\REW(\mA, \mI_j)]} \geq \Omega(\log T).
	\]

	Thus combining this with \refeq{eq:lowerBdOPTFD} we obtain
	\[
			\textstyle \frac{\OPTFD}{\E[\REW(\mA)]} \geq \Omega(\log T) - O\Paren{\frac{\log^{1.5} T}{\sqrt{B}}}.
	\]
	Since $B \geq \Omega\Paren{\log^3 T}$, we get that $\tfrac{\OPTFD}{\E[\REW(\mA)]} \geq \Omega(\log T)$.

\subsection{Best dynamic policy benchmark}
\label{sec:LB-DP}
	We will now prove part (c) of Lemma~\ref{thm:LB-main}. Consider the following construction of the lower-bound example.
		
	\begin{construction}\label{con:LB-DP}
		There is one resource with budget $B$, and two arms, denoted $A_0, A_1$. Arm $A_0$ is the `null arm' that has zero reward and zero consumption. The consumption of arm $A_1$ is $1$ in all rounds. The rewards of $A_1$ are defined as follows. We partition the time into $\tfrac{T}{B}$ phases of duration $B$ each (for simplicity, assume that $B$ divides $T$). We consider $\tfrac{T}{B}$ problem instances; for each instance $\mI_\tau$, $\tau \in \Brac{\tfrac{T}{B}}$ arm $A_1$ has $0$ reward
			in all phases except pahse $\tau$; in phase $\tau$ it has a reward of $1$ in each round.
	\end{construction}
	
	\begin{lemma}
		\label{thm:dynamicPolicy}
		Fix $K=2$ arms, $d=1$ shared resource. Then for every $T \geq 2$, budget $\Omega(1)\leq B \leq O\Paren{T^{1-\alpha}}$ for some $\alpha > 0$ and for every randomized algorithm $\mA$ we have that $\tfrac{\OPTDP}{\E[\REW(\mA)]}$ is at least $\Omega\Paren{\tfrac{T}{B}}$ for the construction~\ref{con:LB-DP}.
		\end{lemma}

	
	\begin{proof}
	From the construction~\ref{con:LB-DP}, we have that the optimal dynamic policy obtains a total reward of $B$ in every instance. We will now show that for any deterministic algorithm $\mA$, $\tfrac{\OPTDP}{\E[\REW(\mA)]}$ is at least $\tfrac{T}{B}$ on any instance chosen uniformly at random from this family $\Set{\mI_{\tau}}_{\tau \in \Brac{ \tfrac{T}{B} }}$. Thus from Yao's lemma~\cite{MR95} we have that for any randomized algorithm $\mA$, $\tfrac{\OPTDP}{\E[\REW(\mA)]}$ is at least $\tfrac{T}{B}$ on at least one instance in this family.
		
		Let $\mA$ denote a deterministic algorithm. We can characterize it by a sequence $\alpha_1, \alpha_2 \LDOTS \alpha_{\tfrac{T}{B}}$ with $\sum_{j \in \Brac{\tfrac{T}{B}}} \alpha_j \leq B$, where $\alpha_{j}$ denotes the number of times arm $A_1$ is chosen in phase $j$. Thus the total reward obtained by $\mA$ on instance $\mI_{\tau}$ is at most $\alpha_{\tau}$. Moreover the expected reward obtained by $\mA$ on a random instance from this family is $\tfrac{B}{T} \sum_{\tau \in \Brac{\tfrac{T}{B}}} \alpha_{\tau}$, since the probability of choosing any instance uniformly at random is $\tfrac{B}{T}$. Note that $\sum_{\tau \in \Brac{\tfrac{T}{B}}} \alpha_{\tau} \leq B$. Thus $\tfrac{\OPTDP}{\E[\REW(\mA)]}$ is at least $\tfrac{T}{B}$.
	\end{proof}


 \subsection{Best fixed arm benchmark}
 \label{sec:LB-FA}
	In this subsection we prove part (d) of Lemma~\ref{thm:LB-main}. We use the following construction for the lower-bound.
	
	\begin{construction}\label{con:LB-DP}
		There is one resource with budget $B$, and $K$ arms denoted by $A_1, A_2 \LDOTS A_K$. Arm $A_K$ is the `null arm' that has zero reward and zero consumption. There are $K$ instances in the family.  In instance $\mI_j$, all arms $A_{j'}$ where $j' > j$ have $0$ reward and $0$ consumption in all time-steps. Consider an instance $\mI_j$ for some $j \in [K-1]$ and an arm $j' \leq j$. Arm $A_{j'}$ has a reward of $\tfrac{1}{K^{K-j'}}$ and consumption of $1$ in all time-steps in phase $j'$ and has a reward of $0$ and consumption of $0$ in every other time-step. Thus the rewards and consumption are bounded in the interval $[0, 1]$ for every arm and every time-step in all instances in this family. 		
	\end{construction}
	
	\begin{lemma}
		\label{thm:bestFixedArmLB}
		Let $T \geq 2$, $2 \leq B \leq T$, $K \geq 3$ be given parameters of the $\AdversarialBwK$ problem. We show that there exists a family of instances with $d=1$ shared resource such that for every randomized algorithm $\mA$ we have $\tfrac{\OPTFA}{\E[\REW(\mA)]}$ is at least $\Omega(K)$ on one of these instances.
	\end{lemma}
	
	\begin{proof}
		First note that the best fixed arm in instance $\mI_j$ is to pick arm $A_j$ which yields a total reward of $\frac{B}{K^{K-j}}$.
		
		Consider a randomized algorithm $\mA$. Observe that in the first $j$ phases, the instances $\mI_{j-1}$ and $\mI_j$ have identical outcome matrices. Thus the expected number of times any arm $A_k$ for $k \in [K]$ is chosen in phases $\Set{1, 2 \LDOTS j}$ should be the same in both the instances. Let $\alpha_k$ denote the expected number of times arm $k$ is played by $\mA$ in phase $k$ on instances $\mI_k, \mI_{k+1} \LDOTS \mI_{K-1}$ \footnote{This has to be the same in all instances since the outcome matrix is identical until phase $k$ in all these instances}. Moreover we have that $\alpha_1 + \alpha_2 \LDOTS \alpha_{K-1} \leq B$.
		
		To show the lower-bound we want to minimize the competitive ratio on every instance for all possible values of $\alpha_1, \alpha_2 \LDOTS \alpha_{K-1}$. For ease of notation denote $r_j := \frac{1}{K^{K-j}}$. Let $\alpha_{\mathcal{B}}$ denote the set of values to $\Set{\alpha_k}_{k \in [K-1]}$ such that $\sum_{k \in [K-1]} \alpha_k \leq B$. Thus, 
		
		\begin{equation}
			\label{eq:bestFixedArmRatio}
			\textstyle	\tfrac{\OPTFA}{\E[\REW(\mA)]} \geq \min_{\alpha_{\mathcal{B}}} \frac{r_k B}{\sum_{j \in [k]} r_j \alpha_j}.
		\end{equation}
		
		The ratio is minimized when all ratios in \refeq{eq:bestFixedArmRatio} are equal. We will show via induction that this yields the following recurrence,
		
		\begin{equation}
			\label{eq:FArecurrence}
			\textstyle \forall k \geq 2 \qquad \alpha_k = \Paren{1-\frac{r_{k-1}}{r_k}} \alpha_1.
		\end{equation}
		
		Combining this with the condition that $\sum_{k \in [K-1]} \alpha_k \leq B$, this yields the condition $\alpha_1 \leq \tfrac{B}{K-\tfrac{1}{K}}$. Moreover the minimizing value in \refeq{eq:bestFixedArmRatio} is $K-\tfrac{1}{K}$ which proves Lemma~\ref{thm:bestFixedArmLB}.
		
		We will now prove the recurrence \refeq{eq:FArecurrence}. Consider the base case with $k=2$. Equalizing the first two terms in \refeq{eq:bestFixedArmRatio} we get
		
		\[
			\textstyle	\frac{r_1 B}{r_1\alpha_1} = \frac{r_2 B}{r_1 \alpha_1 + r_2 \alpha_2}.
		\]
		
		Re-arranging we obtain that $\alpha_2 = \Paren{1- \frac{r_1}{r_2}} \alpha_1$. We will now prove the inductive case. Let the recurrence be true for all $1 \leq k \leq k'$. Consider the case $k=k'+1$. Setting the $k'$ and $k'+1$ ratios in \refeq{eq:bestFixedArmRatio} equal, we obtain
		
		\begin{equation}
			\label{eq:FAinductive}
			\textstyle \frac{r_{k'} B}{\sum_{j \in [k']} r_j \alpha_j} = \frac{r_{k'+1} B}{\sum_{j \in [k' + 1]} r_j \alpha_j}.
		\end{equation}

		
		Moreover from the inductive hypothesis we have $\alpha_j = \Paren{1-\tfrac{r_{j-1}}{r_j}} \alpha_1$ for every $j \leq k'$. Thus we have
		\begin{align*}
				\textstyle \sum_{j \in [k']} r_j \alpha_j & = r_{k'} \alpha_1\\
				\textstyle \sum_{j \in [k' + 1]} r_j \alpha_j &= r_{k'} \alpha_1 + r_{k'+1} \alpha_{k'+1}.
		\end{align*}
	
		Plugging this back in \refeq{eq:FAinductive} we get
		
		\[
				\textstyle \frac{r_{k'} B}{r_{k'} \alpha_1} = \frac{r_{k'+1} B}{r_{k'} \alpha_1 + r_{k'+1} \alpha_{k'+1}}.
		\]
		
		Rearranging we get $\alpha_{k'+1} = \Paren{1-\tfrac{r_k'}{r_{k'+1}}} \alpha_1$. This completes the induction.
	\end{proof}




==> highProbabilityAnalysis.tex <==
\section{Analysis of the high-probability algorithm: proof of Theorem~\ref{thm:AdvBwK-HP}}
\label{sec:analysis-HP}

\newcommand{\ratio}{\term{ratio}}

We prove Theorem~\ref{thm:AdvBwK-HP}, following the plan outlined in the proof sketch. We decompose the analysis into several distinct pieces, present them one by one, and then show how to put them together. Each piece is presented as a lemma, with appropriate notation and intuition; the proofs of these lemmas are deferred to later in this section.

Throughout, we assume that
\begin{align}\label{eq:HP-analysis-assn}
\min\{ \OPTFD, B \} >  \Omega\left( KT^{3/4} \log \tfrac{T}{\delta} \right).
\end{align}
This is without loss of generality, because otherwise the guarantee in Theorem~\ref{thm:AdvBwK-HP} is vacuous. Recall that the primal algorithm $\ALG_1$ satisfies the uniform exploration property \eqref{eq:hp-guess} with parameter $\gamma\geq T^{-1/4}$.

\xhdr{Extended notation.}
To argue about a given phase, we extend some of our notation to refer to arbitrary time intervals, not just $[1,\tau]$. In what follows, fix time interval $[\tau_1,\tau_2]$, and let $\tDelta$$\tau = \tau_2-\tau_1+1$.
Let
\begin{align*}
\bvM_{\Brac{\tau_1, \tau_2}}
    &:= \frac{1}{\tDelta \tau}\,\sum_{t=\tau_1}^{\tau_2}\; \vM_t, \\
\bvM^{\ips}_{\Brac{\tau_1, \tau_2}}
    &:= \frac{1}{\tDelta \tau}\,\sum_{t=\tau_1}^{\tau_2}\; \vM^{\ips}_t
\end{align*}
be, resp., the average outcome matrix and its IPS-estimate on this time interval. Define
\begin{align}
			\OBJ(\Brac{\tau_1, \tau_2}) &:= \tDelta \tau \cdot \OPTLP(\bvM_{\Brac{\tau_1, \tau_2}}, B, \vec{\tDelta}\tau),	\label{eq:OBJ} \\
			\OBJ^{\ips}(\Brac{\tau_1, \tau_2}) &:=  \tDelta\tau \cdot \OPTLP(\bvM^{\ips}_{\Brac{\tau_1, \tau_2}}, B, \vec{\tDelta} \tau). \label{eq:OBJips}
\end{align}
When $\tau_1=1$ we use the short-hand $\OBJ(\tau_2)$ and $\OBJ^{\ips}(\tau_2)$. Recall that
\begin{align}
\OPTLPfull[\tau] &:= \max_{\tau\in [T]}\;\OBJ(\tau). \label{eq:HP-analysis-OPTLPfull}\\
\guess_\tau &:= \max_{\tau\in [T]}\;\OBJ^{\ips}(\tau).
\label{eq:HP-analysis-guess}
\end{align}



\xhdr{IPS estimators are good.}  We argue that, essentially, the guess $\guess_\tau$ is close to $\OPTLPfull[\tau]$ with high probability. More precisely, we prove that $\OBJ(\tau)$ is close to its IPS estimator, for any given $\tau\in [T]$. We will denote the deviation term as
\begin{equation}\label{eq:dev}
	\Dev(\tau) := C_0\Paren{\frac{K\cdot \OBJ(\tau)}{\gamma B} \sqrt{\tau \log \tfrac{1}{\delta}} },
\end{equation}
for a sufficiently large absolute constant $C_0$. Thus,
$\Dev(\tau) \leq O\Paren{ \tfrac{K\,T^{7/4}}{B} \sqrt{\log \tfrac{1}{\delta}} } (:= \Dev(T))$.

In this notation, we characterize the IPS estimators as follows:

%% Commented out a notation.
% Let $R_{0, \delta}(\tau) := \frac{K}{\gamma} \sqrt{2 \tau \log \frac{1}{\delta}}$, $\rho_{\tau} := \Theta\Paren{\frac{1}{B} + \frac{1}{\OBJ(\tau)}}$ and

\begin{lemma}\label{lem:hatLPwithActual}
%Fix round $\tau \in [T]$ such that
%    $\Dev(\tau)\leq \OBJ^2(\tau)/B$.
With probability at least $1-d\delta T$ it holds that
\begin{equation}\label{eq:tailhatLP}
\forall \tau \in [T]\qquad
\OBJ^{\ips}(\tau) - \Dev(\tau)
    \leq \OBJ(\tau)
    \leq \OBJ^{\ips}(\tau) +\Dev(\tau).
\end{equation}
If the event \eqref{eq:tailhatLP} holds, then $\guess_{\tau}$ and
$\OPTLPfull[\tau]$ are indeed close:
\begin{equation}\label{eq:tailhatLP-guess}
\forall \tau \in [T]\qquad
\left| \guess_{\tau} - \OPTLPfull[\tau] \right| \leq \max_{t \in [\tau]} \Dev(t).
\end{equation}
\end{lemma}

The proof only relies on the uniform exploration property \eqref{eq:hp-guess} and the definition of IPS estimators, not on anything that the algorithm does. A somewhat subtle point is to derive concentration on the respective LP-values from concentration of the average outcome matrices.

\xhdr{IPS estimators do not change too fast.}
We use the stopping condition in the algorithm to argue that the IPS estimators $\OBJ^{\ips}(\cdot)$ do not change too fast from one phase to another, in some specific sense. Namely, we compare $\OBJ^{\ips}(\cdot)$ in the first round of any full phase to the guess in the last round of the next phase.

\begin{lemma}\label{lem:HP-stopping}
Consider a full phase in the execution of the algorithm. Let $\tau$ be the first round in this phase, and let $\tau'$ be any round in the next phase. Then
\begin{equation}\label{eq:startToFull}
\frac{1}{\kappa^2} \leq \frac{\OBJ^{\ips}(\tau)}{\guess_{\tau'}} \leq \frac{1}{\kappa} + \frac{K}{\gamma \guess_{\tau'}}.
\end{equation}
\end{lemma}

This Lemma relies only on the stopping condition in the algorithm, $\guess>T_0/\kappa$, and the way  the guess $\guess_\tau$ is expressed in terms of the IPS estimators $\OBJ^{\ips}(\cdot)$, as expressed in \refeq{eq:HP-analysis-guess}. It is irrelevant to this Lemma how the IPS estimators $\OBJ^{\ips}(\cdot)$ are actually defined.

\xhdr{Last full phase offers sufficient rewards.}
Recall that a phase in the execution of the algorithm is called \emph{full} if the stopping condition $\guess_t>T_0/\kappa$ has fired. We focus on the last full phase; let $\tau_{start}, \tau_{end}$ denote the first and last time-steps of this phase. We prove there is enough reward to be collected in this phase.

Let $\tau^*$ denote the maximizer in \refeq{eq:adv-stoppedLP} which we interpret as the \emph{optimal stopping time}. Essentially, we compare the LP value for the time interval $[\tau_{start}, \tau_{end}]$ with the LP value for the time interval $[1,\tau^*]$. The former is expressed as
    $\OBJ(\Brac{\tau_{start}, \tau_{end}})$
and the latter as $\OPTLPfull$. Note $T$ lies in the subsequent phase (so we can apply Lemma~\ref{lem:HP-stopping}).

\begin{lemma}\label{lem:remOPT}
Consider a run of the algorithm such that event \eqref{eq:tailhatLP} holds. Then
\begin{equation}\label{eq:fracRewardsHighP}	
\OBJ(\Brac{\tau_{start}, \tau_{end}}) \geq \left( \frac{1}{\kappa} - \frac{1}{\kappa^2} \right) \OPTLPfull - O(\Dev(T)).
\end{equation}
\end{lemma}


\xhdr{Adversarial analysis of \MainALG.}
Let us plug in the adversarial analysis of \MainALG, as encapsulated in  Lemma~\ref{lm:adv-crux}. We focus on the last full phase in the execution. We interpret it as an execution of algorithm \MainALG with parameters $B_0,T_0$ on an instance of \AdvBwK with budget $B_0$ that starts at round $\tau_{start}$ of the original problem. Let $\guess = \guess_{\tau_{start}}$ be the guess at the first round of the phase. Then the parameters are $B_0 = B/\ratio$ and
    $T_0 = \guess/(\kappa^2\cdot \ratio)$,
where
    $\ratio = \Cel{\log_\kappa T}$.

We apply Lemma~\ref{lm:adv-crux} for round $\sigma=\tau_{end}-\tau_{start}+1$  in the execution of \MainALG. Restated in our notation, $f(\sigma)$ in Lemma~\ref{lm:adv-crux} is
\[ f(\sigma) = \OPTLP(\bvM_{[\tau_{start}, \tau_{end}]}, B_0, \sigma). \]
Thus, we obtain that with probability at least $1-\delta$ we have
\begin{equation} \label{eq:FromAdvGuarantees}
\REW \geq \sum_{t=\tau_{start}}^{\tau_{end}} r_t(a_t) \geq \min\Paren{\frac{\guess}{\lceil \log_{\kappa} T \rceil \kappa^2}, \sigma f(\sigma) - \frac{d \guess}{\lceil \log_{\kappa} T \rceil \kappa^2}} - \reg,
\end{equation}
where the regret term is
    $\reg := R_{1, \delta}(T) + R_{2, \delta}(T)$.

\xhdr{Rescaling the budget.} Since we use rescaled budget $B_0$, it is important to connect the corresponding LP-values to those for the original budget $B$. We have the following general fact (observed in \cite{AgrawalDevanur-ec14}): for any outcome matrix $\vM$, budget $B$, time horizon $T$, and rescaling factor $\psi \in (0, 1]$ it holds that
\begin{align}\label{eq:scaledBudgetOPTVals1}
\OPTLP\Paren{\vM, \psi B, T}
    \geq \psi \cdot \OPTLP\Paren{\vM, B, T}.
%\OPTLP\Paren{\bvM_{\tau}, B_0(1-\psi), \tau}
%    \geq (1- \psi)\cdot \OBJ\Paren{\tau}.
\end{align}
This holds because an optimal solution $\vec{\mu}$ to $\LP_{\vM, B, T}$, the vector $\psi\,\vec{\mu} $ is feasible to $\LP_{\vM, \psi B, T}$.

\xhdr{Putting it all together.} We defer the proofs of Lemma~\ref{lem:hatLPwithActual}, Lemma~\ref{lem:HP-stopping} and Lemma~\ref{lem:remOPT} to the following subsections, and show how to complete the proof of Theorem~\ref{thm:AdvBwK-HP} assuming these Lemmas hold.


\begin{proof}[Proof of Theorem~\ref{thm:AdvBwK-HP}]
Throughout this proof, let us condition on the high-probability events in Lemma~\ref{lem:hatLPwithActual} and \refeq{eq:FromAdvGuarantees}.
Moreover from \refeq{eq:scaledBudgetOPTVals1} we have that $\sigma f(\sigma) \geq  \frac{1}{\ratio} \OBJ(\Brac{\tau_{start}, \tau_{end}})$ since $B_0 = \frac{B}{\ratio}$. Thus combining this with \refeq{eq:FromAdvGuarantees} we get,
		
		\begin{equation}
			\label{eq:HighPSumCond}
			\REW = \sum_{t=\tau_{start}}^{\tau_{end}} r_t(a_t) \geq \frac{1}{\ratio} \min\Paren{\frac{\guess}{\kappa^2}, \OBJ(\Brac{\tau_{start}, \tau_{end}}) - \frac{d \guess}{\kappa^2}} - \reg.
		\end{equation}
		
		Further from Lemma~\ref{lem:remOPT} with $\kappa=d+1$, we can re-write \refeq{eq:HighPSumCond} as
		
		\begin{equation}
			\label{eq:partTwo}
		\textstyle \REW \geq \frac{1}{\ratio} \min\Paren{\frac{\guess}{\kappa^2}, \Paren{\frac{1}{\kappa}-\frac{1}{\kappa^2}} \OPTLPfull - \frac{\guess}{\kappa}} - \reg.
		\end{equation}

		Recall that $\guess$ for the phase $[\tau_{start}, \tau_{end}]$ is $\OBJ^{\ips}(\tau_{start})$. Moreover we have that $T$ lies in the phase immediately after $[\tau_{start}, \tau_{end}]$.

		Thus from \refeq{eq:startToFull} (first inequality below) and \refeq{eq:tailhatLP-guess} (second inequality below) we have,
		
		\begin{equation}
			\label{eq:GhatUpperBound}
			\guess \leq \frac{1}{\kappa} \guess_{T} + \frac{K}{\gamma} \leq \frac{1}{\kappa} \OPTLPfull + O(\Dev(T)).
		\end{equation}

		Likewise we have,
		\begin{equation}
			\label{eq:GhatLowerBound}	
			\guess \geq \OBJ^{\ips}(\tau_{start}) \geq \frac{1}{\kappa^2} \guess_{T} \geq \frac{1}{\kappa^2} \OPTLPfull -O(\Dev(T)),
		\end{equation}
			
		\noindent where the second inequality uses \refeq{eq:startToFull} and the last inequality uses \refeq{eq:tailhatLP}.	 Plugging \refeq{eq:GhatUpperBound} and \refeq{eq:GhatLowerBound} back into \refeq{eq:partTwo} we get,
		
		\begin{equation}
			\label{eq:HighPFinal1}
			\textstyle \REW \geq \frac{1}{\ratio} \min\Paren{\frac{\OPTLPfull}{\kappa^4}, \Paren{\frac{1}{\kappa}-\frac{2}{\kappa^2}} \OPTLPfull} - \reg - O(\Dev(T)).
		\end{equation}
		
		 And from \refeq{eq:adv-stoppedLP} we have $\OPTLPfull \geq \OPTFD$. Plugging this into \refeq{eq:HighPFinal1} we get \refeq{eq:thm:AdvBwK-HP}.
	\end{proof}
		
	\subsection{Proof of Lemma~\ref{lem:HP-stopping}}
		Let $\tau \in [T]$ denote a time-step in the beginning of a phase. Let $\tau' \in [T]$ be a time-step in the next phase. There exists a $j \in \Set{1, 2 \LDOTS \lceil \log_{\kappa} T \rceil}$ such that $\OBJ^{\ips}(\tau) \geq \kappa^j$. Since $\tau$ is the beginning of a phase, this implies that $\OBJ^{\ips}(\tau-1) < \kappa^{j-1}$. Observe that in a single time-step the value of the estimate can increase by at most $\frac{K}{\gamma}$. Thus $\OBJ^{\ips}(\tau) < \kappa^{j-1} + \frac{K}{\gamma}$. Moreover since $\tau'$ belongs to the next phase, we have that $\kappa^{j+1} \leq \guess_{\tau'} \leq \kappa^{j+2}$. Putting these together we get that
		
		\[
				\frac{1}{\kappa^2} \leq \frac{\OBJ^{\ips}(\tau)}{\guess_{\tau'}} \leq \frac{1}{\kappa} + \frac{K}{\gamma \kappa^{j+1}} \leq \frac{1}{\kappa} + \frac{K}{\gamma \guess_{\tau'}}.
		\]
		
	\subsection{Proof of Lemma~\ref{lem:remOPT}}
		We first prove the following property of the optimal solution.
			
		\begin{claim}
				Let $T_1 < T_2$ be any two time-steps. Then,
				\begin{equation}
				\label{eq:diffOPTToFull}	
				\OBJ([T_1, T_2]) \geq \OBJ(T_2)-\OBJ(T_1-1).
			\end{equation}
		\end{claim}
		
		\begin{proof}			
			We prove this claim as follows. Let $\vec{\mu}_{T_2}$ denote the optimal solution to $\LP_{\bvM_{T_2}, B, T_2}$. Since $c_{t, i}(a) \geq 0$ for every $a \in [K]$, $t \in [T]$ and $i \in [d]$ we have
			
			\begin{equation*}
				\textstyle \vec{\mu}_{T_2} \cdot \sum_{t \in [T_2]} \vec{c}_{t, i} \leq B \implies \vec{\mu}_{T_2} \cdot \sum_{t \in [T_1-1]} \vec{c}_{t, i} \leq B.
			\end{equation*}
			
			Thus $\vec{\mu}_{T_2}$ is feasible to $\LP_{\bvM_{T_1-1}, B, T_1-1}$. This implies that $\sum_{t \in [T_1-1]} \vec{\mu}_{T_2} \cdot \vec{r}_t \leq \OBJ(T_1-1)$. Likewise $\vec{\mu}_{T_2}$ is also feasible to $\LP_{\bvM_{[T_1, T_2]}, B, [T_1, T_2]}$.
			
			Therefore we have,
			
			\begin{align}
				\textstyle \OBJ([T_1, T_2]) & \textstyle \geq \sum_{t =T_1}^{T_2} \vec{\mu}_{T_2} \cdot \vec{r}_t \nonumber \\
				& \textstyle = \sum_{t \in [T_2]} \vec{\mu}_{T_2} \cdot \vec{r}_t - \sum_{t \in [T_1-1]} \vec{\mu}_{T_2} \cdot \vec{r}_t \nonumber \\
				& \textstyle = \OBJ(T_2) - \sum_{t \in [T_1-1]} \vec{\mu}_{T_2} \cdot \vec{r}_t \nonumber \\
				& \textstyle \geq \OBJ(T_2) - \OBJ(T_1-1) \nonumber \qedhere
			\end{align}
		\end{proof}	
		
			Consider $\OBJ([\tau_{start}, \tau_{end}])$. From \refeq{eq:diffOPTToFull} we have
			
			\begin{equation}
				\label{eq:applyingTotau}	
				\textstyle \OBJ([\tau_{start}, \tau_{end}]) \geq \OBJ(\tau_{end}) - \OBJ(\tau_{start}-1).
			\end{equation}

			From Lemma~\ref{lem:hatLPwithActual} we can re-write \refeq{eq:applyingTotau} as
			
			\begin{equation}
				\label{eq:tauToips}
				\textstyle \OBJ(\tau_{end}) - \OBJ(\tau_{start}-1) \geq  \OBJ^{\ips}(\tau_{end}) - \OBJ^{\ips}(\tau_{start}-1) - O(\Dev(T)).
			\end{equation}
			
			For some $j \in \lceil \log_{\kappa}(T) \rceil$, at time-step $\tau_{end}$ the value $\guess_t$ exceeds $\kappa^j$ for the first time. Likewise $\guess_t$ exceeds $\kappa^{j-1}$ for the first time at $\tau_{start}$ and is smaller than this value at $\tau_{start}-1$.
			This implies that $\OBJ^{\ips}(\tau_{end}) \geq \kappa^j$ and $\OBJ^{\ips}(\tau_{start}-1) < \kappa^{j-1}$. Therefore \refeq{eq:tauToips} simplifies to
			
			\begin{equation}
				\label{eq:pluggingGuessValues}
			\textstyle \OBJ^{\ips}(\tau_{end}) - \OBJ^{\ips}(\tau_{start}-1) - O(\Dev(T)) \geq \kappa^j - \kappa^{j-1} - O(\Dev(T)).
			\end{equation}
			
			Combining \refeq{eq:pluggingGuessValues}, \refeq{eq:tauToips} and \refeq{eq:applyingTotau} we get
			
			\[
					\textstyle \OBJ([\tau_{start}, \tau_{end}]) \geq 	\kappa^j - \kappa^{j-1} - O(\Dev(T)).
			\]

		Dividing throughout by $\guess_{T}$ and noting that $\guess_T \leq \kappa^{j+1}$ we have,
		\begin{align*}
			\textstyle \frac{\OBJ([\tau_{start}, \tau_{end}])}{\guess_T} & \textstyle \geq \frac{\kappa^{j-1} (\kappa - 1)}{\kappa^{j+1}} - \frac{O(\Dev(T))}{\guess_T}\\
			&\textstyle = \left( \frac{1}{\kappa} - \frac{1}{\kappa^2} \right) - \frac{O(\Dev(T))}{\guess_T}
		\end{align*}
		
		Finally applying Lemma~\ref{lem:hatLPwithActual} to $\guess_T$ we get \refeq{eq:fracRewardsHighP}. This completes the proof of Lemma~\ref{lem:remOPT}.
	
	\subsection{Proof of Lemma~\ref{lem:hatLPwithActual}}
	Recall that for every $t \in [T]$ and $a \in [K]$ we have that $p_t(a)$, the probability that arm $a$ is chosen at time $t$ is at least $\frac{\gamma}{K}$. We now prove Lemma~\ref{lem:highProbabilityDeviations} which relates linear sums of rewards and consumptions computed using the unbiased estimates and the true values. Denote $R_{\gamma, \delta}(\tau) := \frac{K}{\gamma} \sqrt{2 \tau \ln(1/\delta) }$. 
	
	\begin{claim}
			\label{lem:highProbabilityDeviations}
			Let $\delta >0 $, $\gamma > 0$ used by the EXP3.P.1($\gamma$) and time $\tau \in [T]$ be given parameters. Then we have the following statements for any fixed $\vec{z} \in \Delta_K$ each with probability at least $1-\delta$.
			\begin{align}
				&\textstyle \Pr \left[ \left| \sum_{t \in [\tau]} \vec{z} \cdot \Brac{\hat{\vec{r}}_t - \vec{r}_t} \right| > R_{\gamma, \delta}(\tau) \right] \leq \delta \label{eq:rew}\\
				\forall i \in [d] \qquad &\textstyle  \Pr \left[ \left| \sum_{t \in [\tau]} \vec{z} \cdot \Brac{\hat{\vec{c}}_{t, i} - \vec{c}_{t, i}(a)} \right| > R_{\gamma, \delta}(\tau)  \right] \leq \delta \label{eq:cons}
			\end{align}
		\end{claim}
		
			\begin{proof}
			The proof of this follows directly from the invocation of the Azuma-Hoeffding inequality. We will show this for Equation~\eqref{eq:rew}. Define $Y_t := \vec{z}\cdot \Brac{\hat{\vec{r}}_t - \vec{r}_t}$ (like-wise for the lower-tail use $Y_t := \vec{z} \cdot (\vec{r}_t-\hat{\vec{r}}_t)$). Note that this forms a martingale difference sequence since $\mathbb{E}[\vec{z} \cdot (\hat{\vec{r}}_t - \vec{r}_t)~|~\mathcal{H}_{t-1}] = \vec{z} \cdot \Brac{\vec{r}_t-\vec{r}_t} = 0$. Here we used the fact that $\vec{z}$ is not random and fixed before the start of the algorithm. Also we have that $|Y_t| \leq \frac{K}{\gamma}$. Using Lemma~\ref{lem:AzumaHoeffding} we have the desired equation.
		\end{proof}


		
		We will now prove the two inequalities in \refeq{eq:tailhatLP}. We will first prove the first inequality in \refeq{eq:tailhatLP}.
		
		Let $\vec{\mu}^*$ denote the optimal solution to $\OPTLP\Paren{\bvM_{\tau}, B\Paren{1 - \frac{R_{\gamma, \delta}(\tau)}{B} }, \tau}$. Note this is valid whenever $B > \Omega\left( \frac{K}{\gamma} \sqrt{\tau \log \tfrac{1}{\delta}} \right)$. From Equation~\eqref{eq:cons} we have that with probability at least $1-\delta$ for every $ i \in [d]$,
		
		\begin{align}
			\textstyle \sum_{t \in [\tau]} \vec{\mu}^*\cdot \hat{\vec{c}}_{t, i} &\textstyle \leq \sum_{t \in [\tau]} \vec{\mu}^* \cdot \vec{c}_{t, i} + R_{\gamma, \delta}(\tau). \nonumber \\
			&\textstyle \leq B \label{eq:HighPUTResource}
		\end{align}

		\refeq{eq:HighPUTResource} used the fact that $\sum_{t \in [\tau]} \vec{\mu}^* \cdot \vec{c}_{t, i} \leq B\Paren{1 -  R_{\gamma, \delta}(\tau)}$.
		
		
		Using Equation~\eqref{eq:rew}, we have that with probability at least $1-\delta$,
		\begin{equation*}
			\textstyle \sum_{t \in [\tau]} \vec{\mu}^* \cdot \vec{r}_t \leq \sum_{t \in [\tau]} \vec{\mu}^* \cdot \hat{\vec{r}}_t + R_{\gamma, \delta}(\tau).
		\end{equation*}
		
		Using the fact that,
		\[
			\textstyle \sum_{t \in [\tau]} \vec{\mu}^* \cdot \vec{r}_t =  \OPTLP\Paren{\bvM_{\tau}, B\Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}}, \tau},
		\]
		we have the following.
		
		\begin{equation}
			\textstyle \OPTLP\Paren{\bvM_{\tau}, B\Paren{1 - \frac{R_{\gamma, \delta}(\tau)}{B}}, \tau} -  R_{\gamma, \delta}(\tau) \leq \sum_{t \in [\tau]} \vec{\mu}^* \cdot \hat{\vec{r}}_t. \label{eq:HighPUTReward}
		\end{equation}
		
				
		From \refeq{eq:HighPUTResource} we have that $\vec{\mu}^*$ is feasible to $\OPTLP^{\ips}\Paren{\tau}$ and from \refeq{eq:HighPUTReward} this implies that
		
		\begin{equation}
			\label{eq:HighPWTLOPT}
			\textstyle \OBJ^{\ips}\Paren{\tau} \geq \OPTLP\Paren{\bvM_{\tau}, B\Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}}, \tau} -  R_{\gamma, \delta}(\tau).
		\end{equation}

		Finally from \refeq{eq:scaledBudgetOPTVals1} we have
		\begin{equation}
			\label{eq:HighPScaled1}
			\textstyle \OPTLP\Paren{\bvM_{\tau}, B\Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}}, \tau} \geq \Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}} \OBJ\Paren{\tau}.
		\end{equation}
		
		From \refeq{eq:HighPWTLOPT} and \refeq{eq:HighPScaled1} we have
		\[
				\textstyle \OBJ^{\ips}(\tau) \geq \OBJ(\tau) - \underbrace{R_{\gamma, \delta}(\tau)\Paren{1+ \frac{\OBJ(\tau)}{B}}}_{=O\Paren{\frac{K \OBJ(\tau)}{\gamma B} \sqrt{\tau \log \tfrac{1}{\delta}} }},
		\]
		which gives the lower-tail in \refeq{eq:tailhatLP}.

	We will now prove the second inequality in \refeq{eq:tailhatLP} in a similar fashion. Let $\tilde{\vec{\mu}}^*$ denote the optimal solution to
	$\OBJ^{\ips}\Paren{\bvM_{\tau}, B\Paren{1 - \frac{R_{\gamma, \delta}(\tau)}{B} }, \tau}$.
		
	From Equation~\eqref{eq:cons} we have that with probability at least $1-\delta$ for every $ i \in [d]$,
		
		\begin{align}
			\textstyle \sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \vec{c}_{t, i} &\textstyle \leq \sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \hat{\vec{c}}_{t, i} + R_{\gamma, \delta}(\tau). \nonumber \\
			&\textstyle \leq B \label{eq:HighPLTResource}
		\end{align}

		\refeq{eq:HighPLTResource} used the fact that $\sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \hat{\vec{c}}_{t, i} \leq B\Paren{1 -  R_{\gamma, \delta}(\tau)}$.	
		
		Using Equation~\eqref{eq:rew}, we have that with probability at least $1-\delta$,
		\begin{equation*}
			\textstyle \sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \hat{\vec{r}}_t \leq \sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \vec{r}_t + R_{\gamma, \delta}(\tau).
		\end{equation*}
		
		From the fact that
		\[
			\textstyle \sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \hat{\vec{r}}_t =  \OPTLP^{\ips}\Paren{\bvM_{\tau}, B\Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}}, \tau},
		\]
		we get the following.
		
		\begin{equation}
			\textstyle \OPTLP^{\ips}\Paren{\bvM_{\tau}, B\Paren{1 - \frac{R_{\gamma, \delta}(\tau)}{B}}, \tau} -  R_{\gamma, \delta}(\tau) \leq \sum_{t \in [\tau]} \tilde{\vec{\mu}}^* \cdot \vec{r}_t. \label{eq:HighPLTReward}
		\end{equation}

		From \refeq{eq:HighPLTResource} we have that $\tilde{\vec{\mu}}^*_{j}$ is feasible to $\OPTLP\Paren{\tau}$ and from \refeq{eq:HighPLTReward} this implies that
		
		\begin{equation}
			\label{eq:HighPWTUOPT}
			\textstyle \OPTLP^{\ips}\Paren{\bvM_{\tau}, B\Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}}, \tau} \leq \OBJ\Paren{\tau} +  R_{\gamma, \delta}(\tau).
		\end{equation}

		Finally from \refeq{eq:scaledBudgetOPTVals1} we have
		\begin{equation}
			\label{eq:HighPScaled2}
			\textstyle \OPTLP^{\ips}\Paren{\bvM_{\tau}, B\Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}}, \tau} \geq \Paren{1 - \frac{ R_{\gamma, \delta}(\tau)}{B}} \OBJ^{\ips}\Paren{\tau}.
		\end{equation}
		
		Combining \refeq{eq:HighPScaled2} and \refeq{eq:HighPWTUOPT} we get,
		
		\begin{equation}
			\label{eq:HighP2Scaled3}
			\OBJ^{\ips}(\tau) \leq \OBJ(\tau) + \frac{R_{\gamma, \delta}(\tau)}{B - R_{\gamma, \delta}(\tau)} \Paren{\OBJ(\tau) + R_{\gamma, \delta}(\tau)}.	
		\end{equation}
		
		Since $B_0 > 2 R_{\gamma, \delta}(\tau)$ we get,
		
		\[
				\OBJ^{\ips}(\tau) \leq \OBJ(\tau) + \underbrace{ \frac{2R_{\gamma, \delta}(\tau)}{B} \Paren{\OBJ(\tau) + R_{\gamma, \delta}(\tau)}}_{=O\Paren{\frac{K \OBJ(\tau)}{\gamma B} \sqrt{\tau \log \tfrac{1}{\delta}} }},
		\]
		
		and thus we get the upper-tail in \refeq{eq:tailhatLP}.
		
		We will now prove \refeq{eq:tailhatLP-guess}. Recall that $\guess_{\tau} := \max_{t \in [\tau]} \OBJ^{\ips}(t)$. Moreover $\OPTLPfull[\tau] = \max_{t \in [\tau]} \OBJ(t)$.
		
		Consider $\guess_{\tau} - \OPTLPfull[\tau]$. We have,
		
		\begin{align*}
			\guess_{\tau} - \OPTLPfull[\tau] & = \max_{t \in [\tau]} \OBJ^{\ips}(t) - \OPTLPfull[\tau] \\
			& \leq \max_{t \in \tau} (\OBJ(t) + \Dev(t)) - \OPTLPfull[\tau] \\
			& \leq \max_{t \in \tau} \OBJ(t) + \max_{t \in \tau} \Dev(t) - \OPTLPfull[\tau]\\
			& = \max_{t \in \tau} \Dev(t).
		\end{align*}

		Now consider $\OPTLPfull[\tau]-\guess_{\tau}$. We have,
		
		\begin{align*}
			\OPTLPfull[\tau]-\guess_{\tau} &\leq 	\OPTLPfull[\tau] - \max_{t \in [\tau]} (\OBJ(t) - \Dev(t)) \\
			& \leq \OPTLPfull[\tau] - \max_{t \in [\tau]} \OBJ(t) + \max_{t \in [\tau]} \Dev(t) \\
			& = \max_{t \in \tau} \Dev(t).
		\end{align*}


		
		
		
		This completes the proof of Lemma~\ref{lem:hatLPwithActual}.
	


==> related-work.tex <==

\section{Related work}
\label{sec:related}

The literature on regret-minimizing online learning algorithms is vast; see \cite{CesaBL-book,Bubeck-survey12,Hazan-OCO-book} for background. Most relevant are two algorithms for adversarial rewards/costs: Hedge for full feedback \cite{freund1999adaptive}, and EXP3 for bandit feedback \cite{bandits-exp3}; both are based on the weighted majority algorithm from \cite{LittWarm94}.

\StochasticBwK was introduced and optimally solved in \cite{BwK-focs13}. Subsequent work extended these results to soft supply/budget constraints \cite{AgrawalDevanur-ec14}, a more general notion of rewards%
\footnote{The total reward is determined by the time-averaged outcome vector, but can be an arbitrary Lischitz-concave function thereof.}
\cite{AgrawalDevanur-ec14},
combinatorial semi-bandits \cite{Karthik-aistats18}, and contextual bandits \cite{cBwK-colt14,CBwK-colt16,CBwK-nips16}. Several special cases with budget/supply constraints were studied previously:
dynamic pricing \cite{BZ09,DynPricing-ec12,BesbesZeevi-or12,Wang-OR14},
 dynamic procurement \cite{DynProcurement-ec12,Krause-www13} (a version of dynamic pricing where the algorithm is a buyer rather than a seller), dynamic ad allocation \cite{AdsWithBudgets-arxiv13,combes2015bandits}, and a version with a single resource and unlimited time \cite{Gyorgy-ijcai07,TranThanh-aaai10,TranThanh-aaai12,Qin-aaai13}.
 While all this work is on regret minimization,
\cite{GuhaM-icalp09,GuptaKMR-focs11} studied closely related Bayesian formulations.

\StochasticBwK was optimally solved using three different algorithms \cite{BwK-focs13,AgrawalDevanur-ec14}, with extremely technical and delicate analyses. All three algorithms involve inherently `stochastic' techniques such as ``successive elimination" and ``optimism under uncertainty", and do not appear to extend to the adversarial version. One of them, \term{PrimalDualBwK} from \cite{BwK-focs13}, is a primal-dual algorithm superficially similar to ours. Indeed, it decouples into two online learning algorithms: a ``primal" algorithm which chooses among arms, and a ``dual" algorithm similar to ours, which chooses among resources. However, the two algorithms are not playing a repeated game in any meaningful sense, let alone a zero-sum game. The primal algorithm operates under a much richer input: it takes the entire outcome vector for the chosen arm, as well as the ``dual distribution" -- the distribution over resources chosen by the dual algorithm. Further, the primal algorithm is very problem-specific: it interprets the dual distribution as a vector of costs over resources, and chooses arms with largest reward-to-cost ratios, estimated using ``optimism under uncertainty".

Our approach to using regret minimization in games can be traced to \cite{freund1996game,freund1999adaptive} (see Ch. 6 in \cite{SchapireBoosting}), who showed how a repeated zero-sum game played by two agents yields an approximate Nash equilibrium.
%
\OMIT{The framework of regret minimization in games (Lemma~\ref{lem:learningGames} and related results) was introduced in  and has been significant in several ways. On a face value, it is about a game between two agents that run regret-minimizing algorithms. Second, it advances regret minimization as a plausible behavioral model that leads to approximate Nash equilibria. Third, it gives a way compute an approximate Nash equilibrium. }
%
This approach has been used as a unifying algorithmic framework for several  problems: boosting~\cite{freund1996game}, linear programs~\cite{AroraHK}, maximum flow~\cite{Christiano11MaxFlow},
%, connections to differential privacy~\cite{dwork2014algorithmic}
and  convex optimization~\cite{abernethy2017frank,wang2018acceleration}.
While we use a result with the $1/\sqrt{t}$ convergence rate for the equilibrum property, recent literature obtains faster convergence for cumulative payoffs (but not for the equilibrium property) under various assumptions (e.g., \cite{Rakhlin-colt13,Syrgkanis-nips15,Haipeng-colt18}).

	Repeated Lagrangian games, in conjunction with regret minimization in games, have been used in a series of recent papers
\cite{rogers2015inducing,hsu2016jointly,roth2016watch,pmlr-v80-kearns18a,agarwal2018reductions,roth2017multidimensional},
as an algorithmic tool to solve convex optimization problems; application domains range from differential privacy to algorithmic fairness to learning from revealed preferences. All these papers deal with deterministic games (\ie same game matrix in all rounds). Reframing the problem in terms of repeated Lagrangian games is a key technical insight in this work. %particularly in
%\cite{hsu2016jointly,rogers2015inducing,pmlr-v80-kearns18a,agarwal2018reductions}.
Most related to our paper are \cite{roth2016watch,roth2017multidimensional}, where a repeated Lagrangian game is used as a subroutine (the ``inner loop") in an online algorithm; the other papers solve an offline problem. We depart from this prior work in several respects: we use a stochastic game, we deal with some subtleties specific to \StochasticBwK, and we provide a very different analysis for our main results on \AdvBwK, where we cannot rely on the standard machinery.

\OMIT{KARTHIK'S READING REPORT, PLEASE DO NOT REMOVE!
\kaedit{Papers with repeated Lagrangian games \cite{rogers2015inducing,hsu2016jointly,roth2016watch,pmlr-v80-kearns18a,agarwal2018reductions,roth2017multidimensional}.
	\begin{itemize}
		\item Solving an online problem? - \cite{roth2016watch}, \cite{roth2017multidimensional}
		\item Playing on a stochastic game? - None
		\item Using no-regret rather than best-response for the dual? \cite{agarwal2018reductions,pmlr-v80-kearns18a}
		\item Solving the actual problem rather than some subroutine? \cite{hsu2016jointly,rogers2015inducing,pmlr-v80-kearns18a,agarwal2018reductions}.
And all they do, technically, is apply the hammer.
		\item Solving a problem whose relaxation is an LP very much like ours? - Most are general convex programs. Reduction to LP does not make sense in the problem setting.
		\item Doing some adversarial analysis? - Unsure what this means.
		\item Achieving smth optimal-ish? \cite{pmlr-v80-kearns18a,agarwal2018reductions}. Most of these papers do not cite a lower-bound. So I am not sure if its optimal.

	\end{itemize}
}} %\OMIT

% stochastic game, need a dummy resource, optimal only in a regime

	Online packing problems (\eg \cite{BuchbinderNaor09,DevanurJSW-ec11}, see \cite{buchbinder2009design} for a survey) can be seen as a special case of \AdvBwK with a much more permissive feedback model: the algorithm observes full feedback (the outcomes for all actions) before choosing an action. Online packing subsumes various \emph{online matching} problems, including the \emph{AdWords problem} \cite{MSVV07} motivated by ad allocation (see \cite{OnlineMatchingBook} for a survey). While we derive $O(\log T)$ competitive ratio against $\OPTFD$, online packing admits a similar result against $\OPTDP$.%
%%%% Previous footnote
\OMIT{An extension to contextual BwK allows us to treat the full feedback as a context, and compete against the best fixed distribution over policies (see Section~\ref{sec:ext-CB}). The latter benchmark coincides with $\OPTDP$ for both the AdWords and the Online Packing problem. However, for AdWords one can obtain a constant competitive ratio, whereas our results only imply $O(\log T)$ ratio.}

Another related line of work concerns online convex optimization with constraints \cite{mahdavi2012trading,mahdavi2013stochastic,chen2017online,neely2017online,chen2018bandit}. Their setting differs from ours in several important respects. First, the action set is a convex subset of $\R^K$ (and the algorithms rely on the power to choose arbitrary actions in this set). In particular, there is no immediate way to handle discrete action sets.%
\footnote{Unless there is full feedback, in which case one can use a standard reduction whereby actions in online convex optimization correspond to distributions over actions in a $K$-armed bandit problem.}
Second, convexity/concavity is assumed on the rewards and resource consumption.
Third, in addition to bandit feedback, full feedback is observed for the resource consumption, and (in all papers except \cite{chen2018bandit}) one also observes either full feedback on rewards or the rewards gradient around the chosen action. Fourth, their algorithm only needs to satisfy the budget constraints at the time horizon (whereas in BwK the budget constraints hold for all rounds). Fifth, their fixed-distribution benchmark is weaker than ours: essentially, its time-averaged consumption must be small enough at each round $t$. Due to these differences, their setting admits sublinear regret in the adversarial setting, whereas we have a $\Omega(\log T)$ lower bound on the competitive ratio.

Logarithmic competitive ratios are quite common in prior work on approximation algorithms and online algorithms, \eg in the context of the set cover problem \cite{lovasz1975ratio,johnson1974approximation}, buy-at-bulk network design \cite{awerbuch1997buy}, sparsest cut \cite{arora2009expander}, and dial-a-ride problem \cite{charikar1998finite}, the online k-server problem \cite{bansal2011polylogarithmic}, online packing/covering problems \cite{azar2016online}, online set cover \cite{alon2003online}, online network design \cite{umboh2015online}, and online paging \cite{fiat1991competitive}.


\OMIT{ KARTHIK'S READING REPORT, PLEASE DO NOT REMOVE!
\kaedit{notes for related work on Bandit convex optimization.
	All works below have the following setting. At each time, we choose a point $\vec{x}_t$. Then we are shown/receive a loss $f_t(x_t)$ (bandit or full-feedback (varies by work)) and receive cost functions $g_{t,1}, g_{t, 2}, .. g_{t, d}$ (full feedback). The goal is to minimize the total loss $\sum_{t \in [T]} f_t(x_t)$ such that the long-term constraint $\sum_{t \in [T]} g_{t, i} \leq 0$ for every $i \in [d]$. Note that in intermediate time-steps, one can violate the constraints.
	
	This setting differs from BwK in the following ways. First, we only receive bandit feedback in the constraints. Second, in our setting the constraints should be maintained at every time-step. The game stops the first time we violate a constraint. This is critical since, we cannot obtain a sublinear regret with hard constraints, while in their setting they obtain a sub-linear regret. There doesn't seem to be a natural reduction from BwK to their setting. Third, all action sets are convex (and hence continuous). They do not extend to discrete action steps.
	Fourth, the functions $g_{t, i}$ cannot all be positive. This is because, they assume that there exists a feasible solution in hind-sight. Thus, this implies we have both consumption and replenishment of resources.
	
	\begin{itemize}
		\item \cite{chen2017online}. Adversarial setting. Not concurrent work. Full-feedback on the objective.
		\item \cite{neely2017online}. Adversarial setting. Not concurrent work. Full-feedback on the objective. Unpublished.
		\item \cite{mahdavi2012trading}. Adversarial setting. Not concurrent work. Bandit feedback on the objective. The functions $g$ are all known beforehand. They assume that they have access to the gradient of the objective function at each time-step.
		\item  \cite{mahdavi2013stochastic} Stochastic setting. Not concurrent work. Full feedback on the objective. The functions $g$ are all linear.
		\item \cite{chen2018bandit} Adversarial setting. Published 22 May 2018. Bandit feedback on the objective. No gradient assumption. They obtain an estimate to gradient using one point access to the function.
	\end{itemize}
}} %\OMIT

\xhdr{Simultaneous work.}
Two very recent (and yet unpublished) manuscripts have come to our attention after the initial version of this paper has appeared on {\tt arxiv.org}. Rivera et al.~\cite{rivera2018online} consider online convex optimization with knapsacks: essentially, the problem defined in Section~\ref{sec:ext-BCO}, but with full feedback. Focusing on the stochastic version, they design an algorithm similar to \MainALG, and derive a regret bound similar to ours, using a similar analysis. They also claim an extension to bandit feedback, without providing any details (such as precise statement of Lemma~\ref{lem:learningGames} in terms of the regret property \eqref{eq:prelims-regret-weak}).

Rangi et al.~\cite{rangi2018unifying} consider \AdvBwK in the special case when there is only one constrained resource, including time. They attain sublinear regret, \ie a regret bound that is sublinear in $T$. They also assume a known lower bound $c_{\min}>0$ on realized per-round consumption of each resource, and their regret bound scales as $1/c_{\min}$. They also achieve $\text{polylog}(T)$ instance-dependent regret for the stochastic version using the same algorithm (matching results from prior work on the stochastic version). \BwK with only one constrained resource (including time) is a much easier problem, compared to the general case with multiple resources studied in this paper, in the following sense. First, the single-resource version admits much stronger performance guarantees ($\text{polylog}(T)$ vs. $\sqrt{T}$ regret bounds for \StochasticBwK, and sublinear regret vs. approximation ratio for \AdvBwK). Second, the optimal all-knowing time-invariant policy is the best fixed arm, rather than the best fixed distribution over arms.




